Locality Sensitive Hashing in Hyperbolic Space

For a metric space $(X, d)$, a family $\mathcal{H}$ of locality sensitive hash functions is called $(r, cr, p_1, p_2)$ sensitive if a randomly chosen function $h\in \mathcal{H}$ has probability at least $p_1$ (at most $p_2$) to map any $a, b\in X$ in the same hash bucket if $d(a, b)\leq r$ (or $d(a, b)\geq cr$). Locality Sensitive Hashing (LSH) is one of the most popular techniques for approximate nearest-neighbor search in high-dimensional spaces, and has been studied extensively for Hamming, Euclidean, and spherical geometries. An $(r, cr, p_1, p_2)$-sensitive hash function enables approximate nearest neighbor search (i.e., returning a point within distance $cr$ from a query $q$ if there exists a point within distance $r$ from $q$) with space $O(n^{1+\rho})$ and query time $O(n^{\rho})$ where $\rho=\frac{\log 1/p_1}{\log 1/p_2}$. But LSH for hyperbolic spaces $\mathbb{H}^d$ remains largely unexplored. In this work, we present the first LSH construction native to hyperbolic space. For the hyperbolic plane $(d=2)$, we show a construction achieving $\rho \leq 1/c$, based on the hyperplane rounding scheme. For general hyperbolic spaces $(d \geq 3)$, we use dimension reduction from $\mathbb{H}^d$ to $\mathbb{H}^2$ and the 2D hyperbolic LSH to get $\rho \leq 1.59/c$. On the lower bound side, we show that the lower bound on $\rho$ of Euclidean LSH extends to the hyperbolic setting via local isometry, therefore giving $\rho \geq 1/c^2$.

==> legacy/old-proof.tex <==
\subsection{Proof of \Cref{lem:mono-hr}}


Let $f(r) = -\ln(1-\frac{r}{\pi\sinh(R)})$ for $r \in (0,\infty)$ and $g(r) = \frac{f(r)}{f(cr)}$ for some constant $c$. We get $\rho \leq \sup_r\rho(r,c)$ where $\rho(r,c) = g(r)$. A quick observation is that when $r$ is very small, using the standard approximation $\ln(1-x) = -x$, we get $\lim_{r\rightarrow 0}g(r) = 1/c$. In the following lemma, we show that function $g(r)$ is strictly decreasing as $r$ increases, therefore we can conclude $\rho \leq g(0) = 1/c$.

\begin{lemma}
\label{lem:mono-hr}
$g(r)$ is strictly decreasing for some constant $c>1$ and $r\in(0,\infty)$.
\end{lemma}\jie{This is the same as Lemma 1 in [13] -- also mentioned in Lemma 16. So we should skip this lemma}

We prove \Cref{lem:mono-hr} in \Cref{appendix:proof-H2}. 

\begin{proof}
Let the constant $k = 1/(\pi\sinh(R))$, clearly $k > 0$. The function $h(x)$ is given by:
\[ h(x) = \frac{\ln(1 - kx)}{\ln(1 - ckx)} \]
We find the derivative $h'(x)$:
\[ h'(x) = \frac{\left(\frac{-k}{1 - kx}\right) \ln(1 - ckx) - \ln(1 - kx) \left(\frac{-ck}{1 - ckx}\right)}{\ln^2(1 - ckx)} \]
The sign of $h'(x)$ is therefore determined by the sign of its numerator:
\[k \left( \frac{c \ln(1 - kx)}{1 - ckx} - \frac{\ln(1 - ckx)}{1 - kx} \right) \]
It suffices to show that:
\[ \frac{c \ln(1 - kx)}{1 - ckx} \le \frac{\ln(1 - ckx)}{1 - kx} \]
Let $u = 1 - kx$. We can express $1 - ckx$ in terms of $u$:
\[ 1 - ckx = 1 - c(1 - u) = 1 - c + cu \]
Substituting these into the inequality gives:
\[ cu \ln u \le (1 - c + cu) \ln(1 - c + cu) \]
The domain for $u$ is therefore $(1-1/c, 1)$. To prove the inequality, we define an auxiliary function $F(u)$ on this domain:
\[ F(u) = cu \ln u - (1 - c + cu)\ln(1 - c + cu) \]
Our goal is to show that $F(u) \le 0$. The derivative of $F(u)$ is:
\begin{align*}
    F'(u) &= \left[c\ln u + c\right] - \left[c\ln(1-c+cu) + c\right] \\
    &= c[\ln u - \ln(1-c+cu)] = c \ln\left(\frac{u}{1-c+cu}\right)
\end{align*}
For $u < 1$ and $c > 1$, we have $(c-1)(1-u) > 0$, which implies $c-1 > cu-u$, and thus $u > 1-c+cu$. We have $\ln\left(\frac{u}{1-c+cu}\right) > 0$ and $F'(u) > 0$.

This shows that $F(u)$ is a strictly increasing function on its domain. Its maximum value must occur at $F(1) = 0$, therefore $F(u) < 0$ for all $u \in (1-1/c, 1)$. We have shown $h'(x) < 0$ for $x \in (0,\infty)$, which completes the proof.
\end{proof}



==> legacy/oldfiles.tex <==
\section{Our Construction II: $p$-stable Distribution}

\cyd{This probably does not work... two points can be distorted a lot if they are far from the tangent point.}
We now explore if we can adapt the $p$-stable distribution to construct hyperbolic LSH. First, such a distribution is not possible because hyperbolic space $\mathbb{H}^n$ is a Riemannian manifold with constant negative curvature, not a normed vector space. Therefore the two crucial ingredients behind $p$-stable distributions: linearity and translation invariance, break.

However, the tangent space of a Riemannian manifold is a normed vector space. For a point $o\in \mathbb{H}^n$, the \emph{tangent space} $T_o \mathbb{H}^n$ is a Euclidean space $\mathbb{R}^n$. The \emph{logarithmic map} $\log_o:\mathbb{H}^n \to T_o \mathbb{H}^n$ maps $x$ to $X = \log_o(x)$ with $\|X\| = d_\mathbb{H}(o,x)$. This allows us to leverage Euclidean constructions in the tangent space for hyperbolic LSH. A nice property of hyperbolic geometry, is that the hyperbolic distance is locally well-preserved in its tangent space:
\[
\Delta := \|\log_o(x)-\log_o(y)\|
= \left\| \frac{\operatorname{artanh}(\|x\|)}{\|x\|} \, x \;-\; \frac{\operatorname{artanh}(\|y\|)}{\|y\|} \, y \right\|
\]

A \emph{$p$-stable distribution} satisfies: for independent $X_i \sim \mathcal{D}_p$ and coefficients $a_i$,
\[
\sum_i a_i X_i \sim \Big(\sum_i |a_i|^p\Big)^{1/p} X, \quad X\sim \mathcal{D}_p.
\]
Gaussian distributions are 2-stable, Cauchy distributions are 1-stable. $p$-stable distributions are successfully used in Euclidean LSH and achieve $\rho \leq 1/c$. Our hashing scheme, similarly, uses a random Gaussian vector to produce a hash value for each vector of points in the tangent space. Note that now we do not need a bounding ball with radius $R$.

\begin{tbox}
    \textbf{Input:} A point set $P \subseteq \mathbb{H}^n$. Bucket size $w$.
    \begin{enumerate}
        \item Sample a random Gaussian vector $a$, and a real number $b \in (0,w)$.
        \item For each $x\in \mathbb{H}^n$, let $X = \log_o(x)\in T_o \mathbb{H}^n$.
        \item Apply the hash function: $h_{a,b}(x) = \left\lfloor \frac{\langle a, X \rangle + b}{w} \right\rfloor$
        \item Concatenate $k$ independent hashes: $H(x) = (h_{a_1,b_1}(x),\dots,h_{a_k,b_k}(x))$.
    \end{enumerate}
\end{tbox}

We choose $w = r$ and call this algorithm TS-LSH. The focus now is the collision probability and $\rho$. The good thing from $p$-stable distribution, is that the collision probability of $x,y \in \mathbb{H}^n$ depends only on the tangent-space distance $\log_o(x)-\log_o(y)$.
\cyd{Trying to see if the following is true or not.}

\begin{theorem}
For any point set in hyperbolic space $\mathbb{H}^d$, the TS-LSH algorithm achieves $\rho \leq 1/c$ for a $(r,cr,p_1,p_2)$-LSH with high probability. 
% \[
% \rho \le  \left(\frac{\sinh(r/2)}{\sinh(c r/2)}\right)^2 \le \frac{1}{c^2}.
% \]
\end{theorem}

% \begin{lemma}
% For $x,y \in \mathbb{H}^n$ with distance $r$, the collision probability of TS-LSH
% \[
% \Pr[h(x) = h(y)|d_{\mathbb{H}}(x,y) = r] = \int_0^w \frac{1}{\Delta} f\Big(\frac{t}{\Delta}\Big) dt,
% \]
% where $f$ is the pdf of the Gaussian distribution, $\Delta = 2\sinh{r/2}$.
% \end{lemma}
% The probability that two points fall in the same bucket depends on their projection difference $|\langle a, X-Y \rangle| < w$, which scales as $\Delta$.
% \begin{proof}
% In tangent space $T_o \mathbb{H}^n$, $X,Y$ are Euclidean points separated by $\Delta$. The projection along $a$ yields $|\langle a,X-Y\rangle|$ which follows a $p$-stable distribution scaled by $\Delta$. The points collide iff the projected difference is smaller than the bucket width $w$. Integration over the uniform shift $u\in[0,w]$ gives the stated formula.
% \end{proof}

The standard result from Euclidean LSH using $p$-stable distribution~\cite{datar2004locality} shows the collision probability is:
\[
p^\mathbb{E}_1 = \Pr[h_\mathbb{E}(x) = h_\mathbb{E}(y)|d_{\mathbb{E}}(x,y) = r] = 1-2\Phi(-r)-\frac{2}{\sqrt{2\pi}r(1-e^{-r^2/2})},
\]
where function $\Phi$ is the CDF of Gaussian distribution.
% \[
% p_1(r) = \Pr[h(x) = h(y)|d_{\mathbb{H}}(x,y) = r] = \Pr[h_\mathbb{E}(x) = h_\mathbb{E}(y)|d_{\mathbb{E}}(x,y) = 2\sinh(r/2)]
% \]








% \section{Something else}
% A plane can be defined by a non-zero normal vector $u \in \mathbb{R}^3$ and an offset. By the Hyperplane Separation Theorem, a separating plane exists if and only if there is a direction $u$ such that $q$ lies strictly on one side of a plane with normal $u$, while all polyhedra $\{CH_i\}$ lie on the other closed side.

% To simplify the formulation, we can consider a plane that passes through the query point $q$. If any separating plane exists, one can be translated until it touches $q$ while maintaining the separation property. A plane passing through $q$ is defined by its normal vector $u$ as the set of points $x$ satisfying $u \cdot (x - q) = 0$.

% For this plane to separate $q$ from all the polyhedra, every point $p$ belonging to any of the polyhedra $CH_i$ must lie in the same closed half-space. This gives the condition:
% $$u \cdot (p - q) \le 0 \quad \forall p \in \bigcup_{i=1}^{k} CH_i$$

% This single condition must hold for all points in all polyhedra. Since the polyhedra are convex, this condition only needs to be checked for their extreme points. Specifically, for any direction $u$, we only need to verify the condition for the point in $\bigcup CH_i$ that is most extreme in that direction. This leads to the equivalent formulation:
% $$\max_{i=1,...,k} \left( \max_{p \in CH_i} (u \cdot p) \right) \le u \cdot q$$

% Let $p_{ext, i}(u)$ denote the extreme vertex of polyhedron $CH_i$ in the direction $u$. The problem is now reduced to finding if there exists a non-zero vector $u \in \mathbb{R}^3$ that satisfies the following system of $k$ inequalities:
% $$u \cdot p_{ext, i}(u) \le u \cdot q \quad \text{for } i = 1,..., k$$
% This can be rewritten as:
% $$u \cdot (p_{ext, i}(u) - q) \le 0 \quad \text{for } i = 1,..., k$$

% The subproblem is thus a search for a feasible solution $u$ to this system of constraints.

% 2. Linear Programming Formulation
% The feasibility problem described above can be formally expressed as a low-dimensional Linear Program (LP). The variables of the program are the three components of the normal vector $u = (u_x, u_y, u_z)$.

% A separating plane exists if and only if the following LP feasibility problem has a non-trivial solution ($u \neq 0$):

% Find:
% $$u = (u_x, u_y, u_z) \in \mathbb{R}^3$$

% Subject to:
% $$u \cdot (p_{ext, 1}(u) - q) \le 0$$
% $$u \cdot (p_{ext, 2}(u) - q) \le 0$$
% $$\vdots$$
% $$u \cdot (p_{ext, k}(u) - q) \le 0$$
% $$u \neq (0, 0, 0)$$

% This is not a standard linear program because the constraints themselves depend on the variable $u$ (since $p_{ext, i}(u)$ is a function of $u$). This structure defines what is known as an LP-type problem or a generalized linear program. The key feature is that for any fixed direction $u_0$, the constraints become simple linear inequalities that are easy to evaluate.


==> legacy/oldlowerbound.tex <==
\section{Lower Bound}
The lower bound on the performance parameter $\rho$ for LSH of $\ell_p$ metrics has been studied in~\cite{motwani2006lower,o2014optimal}. Theorem 1.3 in~\cite{o2014optimal} stated that for points of  the Hamming cube $\{0, 1\}^d$, an $(r, R, p_1, p_2)$-sensitive LSH of Hamming distance must have \[\rho(c)\geq \frac{e^{2r/d}-1}{e^{2r/d}+1} \]
\cyd{This result is from Motwani [33] not Odonell [35]. And we should probably cite the optimal lb. This loses a factor of 2, but it seems pretty important as it relates to the $c$-approximate NNS.}
Then take $r\approx R/c$, $R\approx d/2$, this gives $2r/d=1/c$ and \[\rho(c)\geq \frac{e^{1/c}-1}{e^{1/c}+1}\geq \frac{e-1}{e+1}\cdot \frac{1}{c}= \Omega(1/c)\]


This lower bound can be used to generate a lower bound of $1/c^p$ for $\ell_p$ distance -- by using $\ell_p$ distance on the same point set. In particular, it shows that LSH for Euclidean distances have $\rho\geq 1/c^2$. We will use the same construction to show a lower bound on $\rho$ for hyperbolic distance. 

We take the Hamming cube $\{0, 1\}^d$ and embed them in $\mathbb{H}^{d+1}$. Specifically, for a point $x_i$ of the Hamming cube, we define $p_i\in \mathbb{H}^{d+1}$ to be $(z, x_i)$ in the half space model, with a very large value of $z$ to be decided later. Now consider the hyperbolic distance of $p_i, p_j$: 
\[d_{\mathbb{H}}(p_i, p_j)=\arccosh(1+\frac{\|x_i-x_j\|^2}{2z^2})\]
For any $0<\eps<1$, we take $z\geq \sqrt{d/2\eps}$. Thus  $\frac{\|x_i-x_j\|^2}{2z^2}\leq \eps$.
Use the generalized power series (Puiseux series) \[\arccosh(1+x)=\sqrt{2}\sum_{t=0}^{\infty}\frac{(-1)^t{2t \choose t}}{(2t+1)8^t}x^{t+1/2}=\sqrt{2x}\left(1-\frac{1}{12}x+\frac{3}{160}x^2 -\frac{5}{896}x^3+\cdots \right)\] 
%\jie{the above expansion formula is from Gemini -- not sure if we can trust it, someone should also verify}  \textcolor{red}{Feng: I checked it using Maple. The formula is correct.  On the other hand, what inequality for arccosh(1+x) are you using? We can probably give a direct proof.}\jie{I added the ineuqality below}
This gives us, for small positive $x$,  \[\sqrt{2x}(1-\frac{1}{12}x)\leq \arccosh(1+x)\leq \sqrt{2x}.\]
We can now bound 
\[\sqrt{\|x_i-x_j\|_1}  (1-\eps/12)\leq  d_{\mathbb{H}}(p_i, p_j)\cdot z\leq \sqrt{\|x_i-x_j\|_1}, \]
where the $\ell_1$ distance (same as the Hamming distance)  $\|x_i-x_j\|_1$ is the same as the squared $\ell_2$ distance $\|x_i-x_j\|_2^2$. 
%\cyd{This is not true right? $\|x_i-x_j\|_1=\|x_i-x_j\|^2$, so by the end you still get $1/c^2$}
Now we build an $(r_h, R_h, p_1, p_2)$-sensitive LSH such that $r_h\cdot z\leq \sqrt{r}$ and $\sqrt{R}(1-\eps/12)\leq R_h\cdot z$. Take $R_h=c_h\cdot r_h$, we have \[\frac{2r}{d}\geq \left(\frac{r_h}{R_h}\right)^2(1-\eps/12)^2=\frac{1}{c_h^2}(1-\eps/12)^2\]
Combining everything, a LSH for $\mathbb{H}^{d+1}$ must have \[\rho(c_h)\geq \frac{e-1}{e+1}\cdot \frac{2r}{d}\geq \frac{e-1}{e+1}\cdot \frac{1}{c_h^2}(1-\eps/12)^2=\Omega(1/c_h^2)\]


% 
